Wasm-R3: Record-Reduce-Replay for Realistic and Standalone WebAssembly Benchmarks

WebAssembly (Wasm for short) brings a new, powerful capability to the web as well as Edge, IoT, and embedded systems. Wasm is a portable, compact binary code format with high performance and robust sandboxing properties. As Wasm applications grow in size and importance, the complex performance characteristics of diverse Wasm engines demand robust, representative benchmarks for proper tuning. Stopgap benchmark suites, such as PolyBenchC and libsodium, continue to be used in the literature, though they are known to be unrepresentative. Porting of more complex suites remains difficult because Wasm lacks many system APIs and extracting real-world Wasm benchmarks from the web is difficult due to complex host interactions. To address this challenge, we introduce Wasm-R3, the first record and replay technique for Wasm. Wasm-R3 transparently injects instrumentation into Wasm modules to record an execution trace from inside the module, then reduces the execution trace via several optimizations, and finally produces a replay module that is executable sandalone without any host environment - on any engine. The benchmarks created by our approach are (i) realistic, because the approach records real-world web applications, (ii) faithful to the original execution, because the replay benchmark includes the unmodified original code, only adding emulation of host interactions, and (iii) standalone, because the replay benchmarks run on any engine. Applying Wasm-R3 to web-based Wasm applications in the wild demonstrates the correctness of our approach as well as the effectiveness of our optimizations, which reduce the recorded traces by 99.53 percent and the size of the replay benchmark by 9.98 percent. We release the resulting benchmark suite of 27 applications, called Wasm-R3-Bench, to the community, to inspire a new generation of realistic and standalone Wasm benchmarks.

==> architecture.tex <==
\subsection{Architecture}
\label{s:architecture}

\begin{figure}[ht]
    \centering
    \includegraphics[width=.9\linewidth]{figures/r3-architecture}
    \caption[Wasm-R3 System Architecture]{\label{fig:r3}\textbf{Wasm-R3 System Architecture.}
    A proxy intercepts the website and adds
    the recording runtime to it. Traces and the original binaries get sent to the server
    which generates the final benchmarks.}
\end{figure}

We give an overview of the Wasm-R3 architecture in figure \ref{fig:overview_arch}.
Wasm-R3 is composed of two phases: recording phase and replay generation phase.
The recording phase is a frontend of Wasm-R3,
which takes a Wasm web application as an input and produces a trace as a result.
The replay generation phase is a backend of Wasm-R3,
which takes the trace as an input and produces the replay benchmarks as a result. 

In recording phase, the Wasm binary of the input web application
is first given as an input to the instrumenter.
The instrumenter instruments each Wasm modules in the app for the recording purpose.
Then, when the application is loaded and user interaction begins, the \textbf{recorder} records
the communication between Wasm and the host environment.
The recorder produces traces, which hold the necessary information to precisely replay the interaction.
The raw trace is optimized to filter out redundant or unnecessary information.

The resulting optimized trace is given as an input to the replay generation phase.
In the first step of the replay generaiton phase,
we generate the replay IR from the input trace.
Then we optimize the raw replay IR to reduce the IR size. 
The replay code generator can produce both JavaScript and Wasm replay codes.
The replay code is packaged with the original Wasm binary to form a replay benchmark.

 
We provide the detailed explanation of each parts in following sections.
In section \ref{s:record}, we explain the  




==> replay_opt.tex <==
\subsubsection{Replay IR Optimization}
\label{s:replay-opt}

\daniel{Since this conceptually happens before the previous section, should we move this section to before the previous section?}
We apply \emph{replay optimization} on the replay IR to reduce the size of replay IR.
Before we generate the output replay benchmark, we reduce the replay IR size so that the size of the replay binary is also reduced.
By reducing the size of replay binary, we solve two issues.
First, we produce valid replay binaries that are accepted by web browser engines.
Production web engines impose a common restriction on the size of functions inside the Wasm binary \footnote{See, e.g., \url{https://github.com/v8/v8/blob/master/src/wasm/wasm-limits.h}.}.
\daniel{(also elsewhere/below:) let's use "production" engines instead of "commercial", since most browsers are free to use.}
By naively translating \verb$Function$ objects in replay IR into Wasm functions, the size of replay functions exceed the function size limit. 
To solve this, we employ replay optimization to reduce number of instructions of each replay functions and produce smaller Wasm replay functions.
Second, we shorten the compilation time of the replay binaries which correlates with the runtime performance of replay benchmark.
A previous study \cite{wizard} have found out that the compilation time of Wasm modules significantly impacts the performance evaluation of a Wasm engine.
Our replay optimization techniques reduce the overall size of the replay binary, we reduce impact of compilation time on the performance evaluation.
\daniel{Didn't we also hyptothesize that merging memory writes could reduce the number of memory operations and thus improve performance? If that's the case, we should also mention that as a reason for the optimization here.}

We describe our two replay optimization techniques: \emph{memory write merge} and \emph{function split}.

\paragraph*{Memory Write Merge Optimization}
By inspecting replay IRs, we found that Wasm often involves writing data to consecutive bytes in the Wasm linear memory.
Inspired by the \wasm{memory.init} instruction executes bulk writes on multiple bytes, we design \emph{memory write merge} optimization that merges multiple \verb$MutateMem$ action on consecutive addresses in a single action.
To represent the bulk write, we introduce a new action \verb$BulkMutateMem$.
\verb$BulkMutateMem$ action has same syntax with \verb$MutateMem$, except the \verb$val$ field is a \verb$I64$ type. 
We translate the \verb$BulkMutateMem$ action into the \wasm{memory.init} Wasm instruction.
In theory, the memory write merge optimization can merge eight \verb$MutateMem$ actions into a single \verb$BulkMutateMem$ action.
\daniel{Why only eight? Seems like an arbitrary limit, can't bulk memory ops write arbitrary numbers of bytes? If there is a good reason why, we should explain it.}

\begin{figure}[h]
\begin{subfigure}[t]{0.5\textwidth}
\begin{lstlisting}[language=Java,numbers=left,label=lst:null1,caption=Replay IR before the optimization]
MutateMem {idx: 0, addr: 0, val: 8}
MutateMem {idx: 0, addr: 1, val: 7}
MutateMem {idx: 0, addr: 2, val: 6}
MutateMem {idx: 0, addr: 3, val: 5}
MutateMem {idx: 0, addr: 4, val: 4}
MutateMem {idx: 0, addr: 5, val: 3}
MutateMem {idx: 0, addr: 6, val: 2}
MutateMem {idx: 0, addr: 7, val: 1}
MutateMem {idx: 0, addr: 8, val: 0}
\end{lstlisting}
\daniel{can we use hex values for the val field to make the matching to the right side clearer?}
\end{subfigure}
~
\begin{subfigure}[t]{0.5\textwidth}
\begin{lstlisting}[language=Java,numbers=left,label=lst:null2,caption=Replay IR after the optimization]
BulkMutateMem {
  idx: 0, 
  addr: 0, 
  val: "\08\07\06\05\04\03\02\01\00"
}
\end{lstlisting}
\end{subfigure}
  \caption{Memory Write Merge Example}
  \label{f:mem-merge}
\end{figure}

Figure \ref{f:mem-merge} illustrates an example of applying memory write merge optimization.
The left-side figure is a part of replay IR before applying the optimization.
It is a sequence of eight \verb$MutateMem$ actions on the consecutive bytes.
By memory write merge optimization, we transform these eight actions into a single action of \verb$BulkMutateMem$ as in the right-side figure.
We merge the eight seperate write values in eight \verb$MutateMem$ actions in to a single, 8-byte value in the \verb$BulkMutateMem$ action.

\paragraph*{Function Split Optimization}
As mentioned earlier, production web browser engines impose a common restriction on the size of a single Wasm function. 
We observed that some \verb$Function$ objects in replay IR have size exceeding the maximum size limit.
These \verb$Function$ objects represent functions frequently called in the Wasm web application execution.
For instance, we observed an untility function that perform the conversion of \verb$float64$ values to integers have millions of actions.

To prevent our output replay binaries from being invalid, we employ \emph{function split optimizations} on such large \verb$Function$ objects.
In function split optimization, we factor out parts of the \verb$Function$ objects into another \verb$Function$ object.
Then we replace the original parts into the call to this \verb$Function$ object.
By setting an appropriate threshold of \verb$Function$ object size, we maintain each \verb$Function$ object size below the maximum Wasm function size limit imposed by the web engines. 
\todo{we do not have replay IR action that can represent this call.}
\todo{i removed the example here. do we need an example here??}
\daniel{No, I don't think we need an example here as a figure, but could we give concrete numbers for typical size thresholds?}

\daniel{Comment for the end of the approach: Do we ever show how the generated replay code (in Wasm) looks like? And give an algorithm or translation rules for how to go from this replay Map[I32, Function] to actual code? I feel this part is missing a bit, and it would be hard for an outsider to understand/replicate our approach without this. In particular, I think the meaning of this I32 and Contexts is not fully clear, and I believe in the implementation we had a "global counter" of some sort, that didn't get mentioned so far, right?}

